Techno-economic criteria to evaluate power flow allocation schemes

We develop novel quantitative techno-economic evaluation criteria for power flow allocation schemes. Such schemes assign which nodes are responsible for which proportion of power flows on a line in a meshed electricity transmission network. As this allocation is, as such, indeterminate, the literature has proposed a number of dedicated schemes. To better understand the implications of applying different schemes, our criteria comprise their (i) fairness, (ii) plausibility, (iii) uniqueness, and (iv) stability. We apply, illustrate, and discuss these criteria for four prominent schemes based on results of a detailed electricity sector model with linear power flow for a German mid-term future case.

==> customcommands.tex <==
%math operators

\newcommand{\E}{\operatorname{E}}
\newcommand\diag[1]{\operatorname{diag}\left(#1\right)}
\newcommand\inv[1]{#1\raisebox{1.15ex}{$\scriptscriptstyle-\!1$}}
\newcommand\abs[1]{\left|#1\right|}
\newcommand\sign[1]{\sigma\left(#1\right)}
\newcommand\M[1]{\begin{bmatrix}#1\end{bmatrix}}

\newcommand{\corr}{\operatorname{corr}}
\newcommand{\<}{\left\langle}
\renewcommand{\>}{\right\rangle}
\newcommand{\BS}{\boldsymbol}
\newcommand{\B}{\mathbf}
\newcommand{\BL}{\textbf}
\newcommand{\re}{\operatorname{Re}}
\newcommand{\identity}{\B{I}}
\newcommand{\Identity}[1]{\identity_\text{#1}}
\newcommand{\ones}{\B{J}}
\newcommand{\Ones}[1]{\ones_\text{#1}}

%basic  
\newcommand{\voltage}{\B{v}}
\newcommand{\current}{\B{i}}
\newcommand{\linecurrent}{\underline{\current}}
\newcommand{\linevoltage}{\underline{\voltage}}
\newcommand{\activepower}{\B{p}}
\newcommand{\reactivepower}{\B{q}}
\newcommand{\voltageangle}{\BS{\theta}}
\newcommand{\power}{\B{s}}
\newcommand{\linepower}{\underline{\B{s}}}
\newcommand{\lineloss}{\underline{\B{s}}^\text{loss}}
\newcommand{\voltagemag}{\hat{\text{v}}}
\newcommand{\injection}{\B{p}}
\newcommand{\flow}{\underline{\B{f}}}
\newcommand{\reactance}{\underline{\B{x}}}
\newcommand{\resistance}{\underline{\B{r}}}
\newcommand{\admittance}{\underline{\B{y}}}
\newcommand{\seriesshuntadmittance}{\underline{\B{y}}^\text{sh}}
\newcommand{\shuntadmittance}{\B{y}^\text{sh}}
\newcommand{\susceptance}{\underline{\B{b}}}
\newcommand{\conductance}{\underline{\B{g}}}
\newcommand{\impedance}{\underline{\B{z}}}
\newcommand{\incidence}{\B{K}}
\newcommand{\laplace}{\B{L}}
\newcommand{\ybus}{\B{Y}}
\newcommand{\zbus}{\B{Z}}
\newcommand{\ptdf}{\B{H}}
\newcommand{\cisf}{\B{H}}
\newcommand{\im}{\textit{j }}
\newcommand{\cycles}{\B{C}}
\newcommand{\Flow}{\B{F}}
\newcommand{\ACflow}{\flow^{\text{AC}}}
\newcommand{\DCflow}{\flow^{\text{DC}}}
\newcommand{\ACcycles}{\cycles^{\text{AC}}}
\newcommand{\DCcycles}{\cycles^{\text{PDC}}}
\newcommand{\Mixedcycles}{\cycles^{\text{mixed}}}
\newcommand{\pseudoimpedance}{\bar{\BS{\omega}}}
\newcommand{\lineefficiency}{\BS{\epsilon}}
\newcommand{\slackconstant}{\B{k}}


%allocation matrices
\newcommand\InjectionMethod[1]{\B{\tilde{P}_{\text{#1}}}} %allocation bus to bus
\newcommand{\allocInjection}{\B{\tilde{P}}} %allocation bus to bus
\newcommand{\allocFlow}{\B{\tilde{F}}} %alternatively \B{T}
\newcommand{\allocbustobus}{\B{A}}
\newcommand{\allocTransaction}{\BS{\mathcal{T}}}


%specific
\newcommand{\Injection}{\B{P}}
\newcommand{\Diff}{\B{D}}
\newcommand{\InjectionMatrix}{\B{G}}
\newcommand{\DirectedIncidence}{\BS{\mathcal{K}}}
\newcommand{\flowloss}{\Delta \flow}

%zbus 
\newcommand{\linevoltageIn}{\linevoltage_{\,\text{in}}}
\newcommand{\linevoltageOut}{\linevoltage_{\,\text{out}}}
\newcommand{\linevoltageInOut}{\linevoltage_{\,\text{in/out}}}

\newcommand{\linepowerIn}{\linepower_{\,\text{in}}}
\newcommand{\linepowerOut}{\linepower_{\,\text{out}}}
\newcommand{\linepowerInOut}{\linepower_{\,\text{in/out}}}

%ap 
\newcommand{\InverseAPInjection}{\BS{\mathcal{J}}}


%editing
\newcommand\note[1]{\textcolor{BrickRed}{#1}}



%costallocation 
\newcommand{\totalcost}{\hat{c}}
\newcommand{\flowcost}{\B{c}}
\newcommand{\restcost}{\text{rest}}
\newcommand{\costperline}{\BS{\gamma}}
\newcommand{\extendedflowcost}{\B{\tilde{\flowcost}}}
\newcommand{\linecapacity}{\B{\Phi}}
\newcommand{\outstandingcost}{\Delta \flowcost}


%infobox for allocation methods
\newcommand{\ConceptBox}[2]{\begin{tcolorbox}[equal height group={#1}A, size=fbox, colback=Apricot!50, colframe=Apricot!80!black, title=\textsc{Concept}] #2 \end{tcolorbox}}

\newcommand{\ApplicationBox}[2]{\begin{tcolorbox}[equal height group={#1}A, size=fbox, colback=Cyan!60, colframe=Cyan!80!black, title=\textsc{Application Case}] #2 \end{tcolorbox}}

\newcommand{\StrengthBox}[2]{\begin{tcolorbox}[equal height group={#1}B, size=fbox, colback=ForestGreen!50, colframe=ForestGreen!80!black!70, title=\textsc{Strength}] #2 \end{tcolorbox}}

\newcommand{\WeaknessBox}[2]{\begin{tcolorbox}[equal height group={#1}B, size=fbox, colback=RedOrange!60, colframe=RedOrange!90!black!80, title=\textsc{Weakness}] #2 \end{tcolorbox}}

\newcommand{\ExtensionBox}[2]{\begin{tcolorbox}[equal height group={#1}C, size=fbox, colback=Lavender!60, colframe=Lavender!80!black, title=\textsc{Extension}] #2
\end{tcolorbox}}

\newenvironment{InfoBox}{\begin{tcbraster}[raster columns=2, boxrule=0mm, arc=0mm, raster right skip= -.0\linewidth, raster left skip = -.0\linewidth, raster row skip = 0.15cm, raster column skip = 0.15cm]}{\vspace{10pt}\end{tcbraster}}

% unbold bold symbol
\newcommand{\unbold}[1]{% 
\begingroup% 
\let\BS\relax% 
\let\B\relax% 
#1 
\endgroup% 
} 
